GI-1.0: A Fast and Scalable Two-level Radiance Caching Scheme for Real-time Global Illumination

Real-time global illumination is key to enabling more dynamic and physically realistic worlds in performance-critical applications such as games or any other applications with real-time constraints.Hardware-accelerated ray tracing in modern GPUs allows arbitrary intersection queries against the geometry, making it possible to evaluate indirect lighting entirely at runtime. However, only a small number of rays can be traced at each pixel to maintain high framerates at ever-increasing image resolutions. Existing solutions, such as probe-based techniques, approximate the irradiance signal at the cost of a few rays per frame but suffer from a lack of details and slow response times to changes in lighting. On the other hand, reservoir-based resampling techniques capture much more details but typically suffer from poorer performance and increased amounts of noise, making them impractical for the current generation of hardware and gaming consoles. To find a balance that achieves high lighting fidelity while maintaining a low runtime cost, we propose a solution that dynamically estimates global illumination without needing any content preprocessing, thus enabling easy integration into existing real-time rendering pipelines.

==> fig/ScreenProbes/comparisonguiding.tex <==
\begin{figure}
\centering
  \begin{subfigure}[b]{0.47\linewidth}
    \includegraphics[width=\linewidth]{fig/ScreenProbes/groundbeforeguiding.png}
    \caption{}
    \label{subfig:gwithout}
  \end{subfigure} 
  \begin{subfigure}[b]{0.47\linewidth}
    \includegraphics[width=\linewidth]{fig/ScreenProbes/groundafterguiding.png}
    \caption{}
    \label{subfig:gwith}
  \end{subfigure}
  \vspace{-5pt}
  \caption{Comparison without  (\protect\subref{subfig:gwithout}) and with (\protect\subref{subfig:gwith}) guiding}
  \label{fig:comparisonguiding}
\end{figure}

==> fig/ScreenProbes/wallstain.tex <==
\begin{figure}
\centering
  \begin{subfigure}[b]{0.47\linewidth}
    \includegraphics[width=\linewidth]{fig/ScreenProbes/vlcsnap-2022-09-15-wall_modified.png}
    % \caption{}
    % \label{fig:blockbase}
  \end{subfigure} 
  \begin{subfigure}[b]{0.47\linewidth}
    \includegraphics[width=\linewidth]{fig/ScreenProbes/vlcsnap-2022-09-15-modified.png}
    % \caption{}
    % \label{fig:complex}
  \end{subfigure}
  \caption{Example of light stains on the walls.}
  \label{fig:wallstains}
\end{figure}

==> fig/irradiance_estimation.tex <==
\begin{figure}
  \centering
  \begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/irradiance_estimation-00.jpg}
    \caption{Screen probes representation}
  \end{subfigure}
  \begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=\linewidth]{fig/irradiance_estimation-01.jpg}
    \caption{Interpolated irradiance}
  \end{subfigure}
  \caption{Per-pixel irradiance evaluated from the probes.}
  \label{fig:irradiance_estimation}
\end{figure}


==> fig/near_far_fields.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{fig/near_far_fields.jpg}
  \caption{Combining near and far-field lighting.}
  \label{fig:near_far_fields}
\end{figure}

